NeuralPLexer3: Accurate Biomolecular Complex Structure Prediction with Flow Models

Structure determination is essential to a mechanistic understanding of diseases and the development of novel therapeutics. Machine-learning-based structure prediction methods have made significant advancements by computationally predicting protein and bioassembly structures from sequences and molecular topology alone. Despite substantial progress in the field, challenges remain to deliver structure prediction models to real-world drug discovery. Here, we present NeuralPLexer3 -- a physics-inspired flow-based generative model that achieves state-of-the-art prediction accuracy on key biomolecular interaction types and improves training and sampling efficiency compared to its predecessors and alternative methodologies. Examined through newly developed benchmarking strategies, NeuralPLexer3 excels in vital areas that are crucial to structure-based drug design, such as physical validity and ligand-induced conformational changes.

==> tables.tex <==


\begin{table}
     \footnotesize
     \begin{center}
     \makebox[\textwidth][c]{
    \begin{tabular}{lcccccc|cccccc}
    
    \toprule
     &\multicolumn{6}{c}{Top-1 Ligand RMSD} & \multicolumn{5}{c}{Top-5 Ligand RMSD}\\
    %  \cmidrule{2-9}
     &\multicolumn{3}{c}{Percentiles (\AA) $\downarrow$} & \multicolumn{2}{c}{Below threshold (\%) $\uparrow$} & Average  & \multicolumn{3}{c}{Percentiles (\AA) $\downarrow$} & \multicolumn{2}{c}{Below threshold (\%) $\uparrow$}\\
    % \cmidrule{3-16} 
    
    \textbf{Methods} & 25th & 50th & 75th & 5 \AA{}  &  2 \AA{} & GPU time (s) & 25th & 50th & 75th & 5 \AA{}  &  2 \AA{} \\
    \midrule
    P2Rank+GNINA~\cite{corso2022diffdock} & 1.7 & 5.5 & 15.9 & 47.8 & 28.8 & 127 & 1.7 & 5.5 & 15.9 & 47.8 & 28.8  \\ 
    DiffDock~\cite{corso2022diffdock} & 1.4 & 3.3 & 7.3 & 63.2 & 38.2 & 40 & 1.2 & 2.4 & 5.0 & 75.5 & 44.7 \\ 
    PointSite+Uni-dock~\cite{yu2023deep} & - & 5.54$\pm$0.46 & - & - & 32.1$\pm$0.9 & - & - & 2.52$\pm$0.18 & - & - & 46.1$\pm$0.69  \\ 
    DiffDock+Uni-dock~\cite{yu2023deep} & - & 4.14$\pm$0.07 & - & - & 38.9$\pm$0.2 & - & - & 1.93$\pm$0.12 & - & - & 51.1$\pm$1.1  \\ 
    NeuralPLexer (ours) & \textbf{1.37$\pm$0.04} &  \textbf{2.85$\pm$0.07} & \textbf{5.97$\pm$0.17} & \textbf{69.7$\pm$0.9} & \textbf{39.7$\pm$0.8} & \textbf{2.1} & 1.06$\pm$0.02 & 2.27$\pm$0.06 & 4.68$\pm$0.11 & 76.6$\pm$0.7 & 46.8$\pm$0.8 \\ 
    \bottomrule
    \end{tabular}}
    \end{center}
    \caption{Summary of performance statistics for rigid receptor blind protein-ligand docking on the PDBBind2020 benchmark. Statistics for the baseline methods are obtained from the sources referenced in their respective rows. Additional computational and timing details are available in Supplementary Information J. Bold-formatted numbers represent the best-performing result on each performance metric. Note that the top-5 statistics reported by baseline methods may depend on their pose selection schemes; the NeuralPLexer top-5 results are computed using 5 randomly sampled poses per protein-ligand pair, and thus should be considered a success rate lower bound. Standard deviations are obtained by performing bootstrapping analysis on 32 independent predictions. }
    \label{tab:table1}
\end{table}
